Differential Privacy Dynamics of Langevin Diffusion and Noisy Gradient Descent

What is the information leakage of an iterative randomized learning algorithm about its training data, when the internal state of the algorithm is \emph{private}? How much is the contribution of each specific training epoch to the information leakage through the released model? We study this problem for noisy gradient descent algorithms, and model the \emph{dynamics} of R\'enyi differential privacy loss throughout the training process. Our analysis traces a provably \emph{tight} bound on the R\'enyi divergence between the pair of probability distributions over parameters of models trained on neighboring datasets. We prove that the privacy loss converges exponentially fast, for smooth and strongly convex loss functions, which is a significant improvement over composition theorems (which over-estimate the privacy loss by upper-bounding its total value over all intermediate gradient computations). For Lipschitz, smooth, and strongly convex loss functions, we prove optimal utility with a small gradient complexity for noisy gradient descent algorithms.

==> appendices/LSI.tex <==
\section{Proof techniques for log-Sobolev inequality}

\label{sec:appendixLSI}

As mentioned before, the literature on LSI is rich with a variety of techniques used to prove this inequality for several kinds of distributions. To prove that LSI holds for the tracing diffusion, we rely on the following two lemmas that show Lipschitz transformation and Gaussian perturbation of a probability distribution preserve its LSI property.

\begin{lemma}[LSI under Lipschitz transformation~\cite{ledoux2001concentration}]
    \label{lem:lip_lsi}
    %
    Suppose a probability distribution $\rhO$ on $\thetaspace$ satisfies LSI with constant~$\alp > 0$.  Let $T:\thetaspace \rightarrow \thetaspace$ be a differentiable and $\lip$-Lipschitz transformation. The push-forward distribution~$T_{\#\rhO}$, representing $T(\thet)$ when $\thet \sim \rhO$, satisfies LSI with constant~$\frac{\alp}{\lip^2}$.
\end{lemma}

\begin{lemma}[LSI under Gaussian convolution~\cite{ledoux2001concentration}]
    \label{lem:gaus_conv_lsi}
    %
    Suppose a probability distribution $\rhO$ on $\thetaspace$ satisfies LSI with constant~${\alp > 0}$.  For $t>0$, the probability distribution $\rhO * \Gaus{0}{2t\Id}$ satisfies LSI with constant~$\left(\frac{1}{\alp} + 2t\right)^{-1}$. A special case of this is that $\Gaus{0}{2t\Id}$ satisfies LSI with constant~$\frac{1}{2t}$.
\end{lemma}


\begin{replemma}{lem:iso_convex}
    %
    If loss function $\loss{\x}{\ptheta}$ is $\cvx$-strongly convex and $\smh$-smooth over a closed convex set $\C$, the step-size is ${\step < \frac{1}{\smh}}$, and initial distribution is $\thet_{0} \sim \proj{\C}{\Gaus{0}{\frac{2\tnoise^2}{\cvx}\Id}}$, then the distribution of tracing diffusion~$\thet_t$ for noisy GD satisfies $\alp$-LSI for any $t\geq0$ with 
    %
    \begin{equation*}
        \alp=\frac{\lam}{2\sig^2}.
    \end{equation*}
 \end{replemma}
 
 \begin{proof}
     For any $\D \in \Domain$, and $0\leq s\leq\step$, define the update step in \alg{alg:noisygd} to be the mapping ${T(\ptheta)=\proj{\C}{ T_1(\ptheta)}}$, where ${T_1(\ptheta)=\ptheta- s\graD{\Loss_\D(\ptheta)}}$. We first show that $T_1$ is $(1-s\cvx)$-Lipschitz. For any $w, v \in \thetaspace$, we have
     \begin{align*}
         T_1(w)-T_1(v) &= w-v-s(\graD{\Loss_\D(w)}-\graD{\Loss_\D(v)})\\
         &=w-v- s\hesS{\Loss_\D(z)}(w-v) \tag{for some $z \in \thetaspace$ due to M.V.T}\\
         &=(I-s\hesS{\Loss_\D(z)})(w-v)
     \end{align*}  
     By convexity and $\smh$-smoothness, $\hesS{\Loss_\D}$ has eigenvalue in $[\cvx,\smh]$. Since $s \leq \step\leq \frac{1}{\smh}$, all eigenvalues of $(I- s\graD{\Loss_\D})$ is in $[0,1-s\cvx]$, so $T_1$ is $(1-s\cvx)$-Lipshitz. 
     
     Now, using induction we prove $\rhO_t$ statisfies $\alp$-LSI for $\alp=\frac{\cvx}{2\tnoise^2}$ for any $t \geq 0$. 
     
     {\bf Base step:} Being a Gaussian with variance $\frac{\cvx}{2\tnoise^2}$, $\rhO_0$ satisfies $\alp$-LSI with the given constant as per lemma \ref{lem:gaus_conv_lsi}.    
 
     {\bf Induction step:} Suppose $\rhO_{\step\kk}$ satisfies $\alp$-LSI with the above constant for some $k \in \N$. Distribution $\rhO_{t}$ for ${\step \kk \leq t < \step (\kk+1)}$ is same as $T$ pushover distribution plus gaussian noise distribution, i.e.  ${\rhO_t = \rhO_{\step \kk}}_{\# T} * \Gaus{0}{2s\tnoise^2\Id}$ for $s = t - \step \kk$. Using lemma \ref{lem:lip_lsi} and \ref{lem:gaus_conv_lsi}, we get
     $\left( \frac{\alp}{(1 - s\cvx)^2 + 2s\tnoise^2\alp} \right)$-LSI for $\rhO_t$.
     Since $s \leq \step \leq \frac{1}{\cvx}$, we have
     \begin{equation*}
         (1-s\cvx)^2 + 2s\tnoise^2\alp \leq 1 - s\cvx + 2s\tnoise^2\alp = 1.
     \end{equation*}
     So for $\eta\kk\leq t<\eta(\kk+1)$, $\rhO_{t}$ satisfies $\alp'$-LSI with constant $\alp' \geq \alp$, which by definition also satisfies $\alp$-LSI.
     For $t=\eta(\kk+1)$, $p_{(k+1)\eta}=$ is same as projected $T$ pushover distribution plus gaussian noise distribution. We've already proved that $T$ pushover distribution plus gaussian noise distribution still satisfies $\alp$-LSI. And since projection is a 
     $1$-Lipschitz map, by Lemma \ref{lem:lip_lsi}, it preserves $\alp$-LSI. So distribution $p_{(k+1)\eta}$ satisfies $\alp$-LSI.
 \end{proof}

==> appendices/NoisyGD_proofs.tex <==
\section{Proofs for privacy analysis of Noisy GD}
\label{sec:noisygdproof}

\begin{replemma}{lem:GDupdate_fokker}
    For SDE \eqr{eqn:discreteSDE}, the equivalent Fokker-Planck equation at time $\step\kk \leq t < \step(\kk+1)$ is
    \begin{equation}
        \doh{\rhO_t(\ptheta)}{t} = \divR{\left(\rhO_t(\ptheta)\Expec{\ptheta_\kk \sim \rhO_{\step\kk|t}}
        {\graD{\Loss_\D(\ptheta_\kk)|\ptheta}}\right)} + \tnoise^2\lapL{\rhO_t(\ptheta)},
    \end{equation}
    where the conditional distribution is defined as
    \begin{equation}
        \rhO_{\step\kk|t}(\ptheta|\ptheta') = \frac{\rhO_{\step\kk,t}(\ptheta, \ptheta')}{\rhO_t(\ptheta')}.
    \end{equation}
\end{replemma}

\begin{proof}
    Recall that conditionals of joint distribution $\rhO_{\step\kk,t}$ is 
    \begin{equation}
        \label{eqn:marg_cond}
        \rhO_{\step\kk,t}(\ptheta', \ptheta) = \rhO_{\step\kk}(\ptheta') \rhO_{t|\step\kk}(\ptheta|\ptheta') = \rhO_{t}(\ptheta) \rhO_{\step\kk|t}(\ptheta'|\ptheta).
    \end{equation}
    Marginalising away $\ptheta'$ in \eqr{eqn:marg_cond} and taking partial derivative w.r.t. $t$, we obtain the following.
    \begin{align*}
        &\doh{\rhO_t(\ptheta)}{t} = \int_{\thetaspace} \doh{\rhO_{t|\step\kk}(\ptheta|\ptheta')}{t}\rhO_{\step\kk}(\ptheta') \dif{\ptheta'} \\
        &\quad= \int_{\thetaspace} \left(\divR{\left(\rhO_{\step\kk,t}(\ptheta',\ptheta)\graD{\Loss_\D(\ptheta')}\right)} + \tnoise^2\lapL{\rhO_{\step\kk, t}(\ptheta', \ptheta)}\right) \dif{\ptheta'} \\
        &\quad=\divR{\left(\rhO_t(\ptheta)\int_{\thetaspace} \rhO_{\step\kk|t}(\ptheta'|\ptheta) \graD{\Loss_\D(\ptheta')\dif{\ptheta'}}\right)} + \tnoise^2\lapL{\rhO_t(\ptheta)} \\
        &\quad=\divR{\left(\rhO_t(\ptheta)\Expec{\ptheta' \sim \rhO_{\step\kk|t}}{\graD{\Loss_\D(\ptheta')}|\ptheta}\right)} + \tnoise^2\lapL{\rhO_t(\ptheta)}
    \end{align*}
\end{proof}

\begin{replemma}{lem:new_delayed_loss_diff}
    Let $\loss{\x}{\ptheta}$ be a $\be$-smooth loss function on closed convex set $\C$, with a finite total gradient sensitivity $\sen{\g}$, then for coupled tracing diffusions $\{\thet_t\}_{t\geq0}$ and $\{\thet_t'\}_{t\geq0}$ on neighboring datasets $\D, \D' \in \Domain$, under loss ${\smaloss{\x}{\ptheta}}$ and noise variance $\tnoise^2$, 
    the gradient sensitivity of conditionally expected loss is bounded by
    \begin{align}
        \Big\Vert\Expec{\ptheta_\kk\sim p_{\eta\kk|t}}{\graD{\Loss_{\D}(\ptheta_\kk)}\vert\ptheta} - &\Expec{\ptheta_\kk'\sim p'_{\eta\kk|t}}{\graD{\Loss_{\D'}(\ptheta_{\kk}')}\vert\ptheta}\Big\Vert_2^2 \leq \frac{S_g^2}{n^2(1-\step\be)^2}.
    \end{align}
\end{replemma}

\begin{proof}
    By definition of coupled tracing diffusion and \eqr{eqn:soldiscreteSDE}, we have for any $\tnoise^2$ and $\step$, the random variables $\thet_{\step\kk}, \thet_{\step\kk}', \thet_t, \thet_t'$ satisfy
    \begin{align}
        \label{eqn:new_delayed_update}
        \thet_{\step\kk} - (t-\step\kk) \graD{\Loss_\D(\thet_{\step\kk})} + \sqrt{2t\tnoise^2}\Z = \thet_t, \\
        \thet_{\step\kk}' - (t-\step\kk) \graD{\Loss_{\D'}(\thet_{\step\kk}')} + \sqrt{2t\tnoise^2}\Z' = \thet_t',
    \end{align}
    where $\Z, \Z' \sim \Gaus{0}{\Id}$, and $\kk$ is an integer s.t. ${\step\kk \leq t \leq \step(\kk+1)}$.

    We define the gradient descent update without noise on datasets $\D, \D'$ to be
    \begin{align}
        \phi(\ptheta)=I(\ptheta)-(t-\eta\kk)\nabla\Loss_{\D}(\ptheta), \\
        \phi'(\ptheta)=I(\ptheta)-(t-\eta\kk)\nabla\Loss_{\D'}(\ptheta),
    \end{align}
    where $I(\ptheta) = \ptheta$. By $\be$-smoothness of $\Loss_{\D}(\ptheta)$ and $\Loss_{\D'}(\ptheta)$, when $\be(t-\step\kk)<1$, for any $\ptheta_1,\ptheta_2\in\thetaspace$, we have
    \begin{align}
        \label{eqn:bilip}
        1-\eta\beta& \leq \frac{\norm{\phi(\ptheta_1)-\phi(\ptheta_2)}}{\norm{\ptheta_1-\ptheta_2}} \leq 1+\eta\beta,
    \end{align}
    and
    \begin{align}
        \label{eqn:bilip_1}
        1-\eta\beta & \leq \frac{\norm{\phi'(\ptheta_1)-\phi'(\ptheta_2)}}{\norm{\ptheta_1-\ptheta_2}} \leq 1+\eta\beta.
    \end{align}

    \textbf{Claim: $\phi$ and $\phi'$ is bijective.}

    \textbf{Proof:} \begin{enumerate}
        \item By \eqr{eqn:bilip}, $\norm{\phi(\ptheta_1)-\phi(\ptheta_2)}\geq (1-\eta\beta)\norm{\ptheta_1-\ptheta_2}$, $\therefore\phi$ is injective.
        \item Now we prove $\phi$ is surjective by proving its range $\phi(\thetaspace)=\thetaspace$.
        \begin{enumerate}
            \item We first prove $\phi(\thetaspace)$ is closed in $\thetaspace$. We only need to prove that any Cauchy sequence in $\phi(\thetaspace)$ converges to a point in $\phi(\thetaspace)$.  For any  $\{\phi(x_n)\}$ that is a cauchy sequence in $\phi(\thetaspace)$, by \eqr{eqn:bilip}, $\{x_n\}$ is also a cauchy sequence in $\thetaspace$, therefore ${\exists x\in\thetaspace}$, s.t. ${lim_{n\rightarrow\infty}x_n=x}$. By continuity of mapping $\phi$, ${lim_{n\rightarrow \infty}\phi(x_n)=\phi(lim_{n\rightarrow\infty}x_n)\in \mathbb{R}^d}$, therefore $\phi(\thetaspace)$ is closed.
            \item We then prove $\phi(\thetaspace)$ is open in $\thetaspace$. Since $\phi:\thetaspace\rightarrow\phi(\thetaspace)$ is injective continuous map, by invariance of domain theorem in topology, $\phi(\thetaspace)$ is an open set in $\thetaspace$.
            \item Since $\phi(\thetaspace)$ is closed and open in $\thetaspace$ and it's nonempty, we conclude that $\phi(\thetaspace)=\thetaspace$. That is $\phi$ is surjective. 
        \end{enumerate}
        \item Therefore $\phi$ is bijective.  Similarly we can prove $\phi'$ is bijective.
    \end{enumerate}
    
    Now we can define inverse $\psi=\phi^{-1}$, $\psi'=\phi'^{-1}$. 
    
    For any $\ptheta_3,\ptheta_4\in\thetaspace$, by \eqr{eqn:bilip}, we have
    \begin{align}
        \label{eqn:inverbilip}
        \frac{1}{1+\step\be}&\leq\frac{\norm{\psi(\ptheta_3)-\psi(\ptheta_4)}}{\norm{\ptheta_3-\ptheta_4}} \leq \frac{1}{1-\step\be},\\
        \frac{1}{1+\step\be}&\leq\frac{\norm{\psi'(\ptheta_3)-\psi'(\ptheta_4)}}{\norm{\ptheta_3-\ptheta_4}}\leq \frac{1}{1-\step\be}.
    \end{align}
    Suppose $\xi(\ptheta)=\phi'(\psi(\ptheta))$, then $\psi(\ptheta)=\psi'(\xi(\ptheta))$ and
    \begin{align}
        \xi(\ptheta)-\ptheta&=\phi'(\psi(\ptheta))-\phi(\psi(\ptheta))\\
        &=(t-\eta\kk)(\graD{\Loss_{\D'}(\psi(\ptheta))}-\graD{\Loss_{\D}(\psi(\ptheta))}).
    \end{align}
    Therefore,
    \begin{equation}
        \label{eqn:xirelation}\norm{\xi(\ptheta)-\ptheta}\leq (t-\eta\kk)\ \underset{\ptheta\in\thetaspace}{max}\ \norm{\graD{\Loss_{\D}(\ptheta)}-\graD{\Loss_{\D'}(\ptheta)}}
    \end{equation}
    Let the conditional gradient expectation $G(\ptheta) = \Expec{\ptheta_\kk\sim p_{\eta\kk|t}}{\graD{\Loss_{\D}(\ptheta_\kk)}\vert\ptheta} = \Expec{}{\graD{\Loss_{\D}(\thet_{\step\kk})}\vert \thet_t= \ptheta}$ be a function of $\ptheta$, and let ${G'(\ptheta) = \Expec{\ptheta_\kk'\sim p'_{\eta\kk|t}}{\graD{\Loss_{\D'}(\ptheta_{\kk}')}\vert\ptheta} = \Expec{}{\graD{\Loss_{\D'}(\thet_{\step\kk}')}\vert\thet_t'=\ptheta}}$. By \eqr{eqn:new_delayed_update} and~$\Expec{}{Z\vert\ptheta_t}=\Expec{}{Z'\vert\ptheta_t}$,  we have
    \begin{align*}  
        G(\ptheta) - G'(\ptheta)&=\frac{1}{t-\step\kk}\Expec{}{\thet_{\step\kk}-\thet_{\step\kk}'\vert\thet_t=\thet_t'=\ptheta}\\
        &=\frac{1}{t-\step\kk}\mathbb{E}[\psi(\ptheta+\sqrt{2\eta\sig^2}\Z)\\
        &\quad -\psi'(\ptheta+\sqrt{2\eta\sig^2}\Z')]\\
        &=\frac{1}{t-\eta\kk}\mathbb{E}[\psi'(\xi(\ptheta+\sqrt{2\step\sig^2}\Z))\\
        &\quad -\psi'(\ptheta+\sqrt{2\step\sig^2}\Z')]
    \end{align*}
    Note that since $\Z$ and $\Z'$ are i.i.d. gaussian standard noise, we can write the above as 
    \begin{align*}
        G(\ptheta) - G'(\ptheta)&=\frac{1}{t-\eta\kk}\mathbb{E}[\psi'(\xi(\ptheta+\sqrt{2\step\sig^2}\Z))\\
        &\quad -\psi'(\ptheta+\sqrt{2\step\sig^2}\Z)]
    \end{align*}
    where $\Z$ is standard gaussian noise. Note that
    \begin{align*}    
        \norm{\psi'(\xi(\ptheta))-\psi'(\ptheta)}
        &\leq \frac{\norm{\xi(\ptheta)-\ptheta}}{1-\step\be}\quad \tag{by \eqr{eqn:inverbilip}}\\
        &\leq\frac{(t-\eta\kk)\ \underset{\ptheta\in\thetaspace}{max}\ \norm{\graD{\Loss_{\D}(\ptheta)}-\graD{\Loss_{\D'}(\ptheta)}}}{1-\step\beta}. \tag{by \eqr{eqn:xirelation}}
    \end{align*}
    Therefore, we have for any $\theta\in\mathbb{R}^d$
    \begin{align*}
        \norm{G(\ptheta) - G'(\ptheta)}&\leq \frac{\norm{\graD{\Loss_{\D}(\ptheta+\sqrt{2\step\sig^2 } Z )}-\graD{ \Loss_{\D'}( \ptheta+\sqrt{2\step\sig^2}Z ) }}}{1-\eta\beta}\\
        \text{By definition of $S_g$}\quad&\leq \frac{S_g}{n(1-\eta\be)}.
    \end{align*}
\end{proof}



\begin{lemma}[ Rate of R\'enyi privacy loss ]
    \label{lem:marginalrenyidiscrete}
    %
    Let $\{\thet_t\}_{t\geq 0}$ and $\{\thet_t'\}_{t\geq 0}$ be the coupled tracing 
    diffusions on neighboring datasets $\D,\D'\in\Domain$ for noisy GD under loss $\loss{\x}{\ptheta}$, noise variance $\sig^2$ and step-size $\step$.
    If loss function $\loss{\x}{\ptheta}$ is $\smh$-smooth, total gradient $g(\ptheta;\D)$ has finite sensitivity $\sen{\g}$, and the update step-size $\step<\frac{1}{\be}$, then for any $t \geq 0$, the rate of R\'enyi privacy loss of the tracing diffusion is upper bounded by
    %
    \begin{align} 
        \negthickspace\negmedspace\doh{\Ren{\q}{\thet_t}{\thet_t'}}{t} \leq 
        \frac{1}{\gamma}\frac{\q \sen{\g}^2}{4\tnoise^2\size^2(1-\step\be)^2}-(1-\gamma)\frac{\tnoise^2\q}{2}\frac{\Gren{\q}{\thet_t}{\thet_t'}}{\Fren{\q}{\thet_t}{\thet_t'}}.
    \end{align}
    where $\gamma>0$ is a tuning parameter that we can fix arbitrarily according to our need.
\end{lemma}
    
\begin{proof}
    For brevity, let the functions ${R(\q,t)=\Ren{\q}{\rhO_{t}}{\rhO_{t}'}}$, ${E(\q,t)=\Fren{\q}{\rhO_{t}}{\rhO_{t}'}}$, and ${I(\q,t)=\Gren{\q}{\rhO_{t}}{\rhO_{t}'}}$. Following the same strategy as in proof of Lemma \ref{lem:marginalrenyi}, we can decompose $\doh{E(\q,t)}{t}$ using the Fokker-Planck equation \eqr{eqn:GDupdate_fokker} into
    \begin{equation*}
        \doh{E(\q,t)}{t} = F_1 + F_2,
    \end{equation*}
    where $F_1 = -\tnoise^2 \q(\q-1) I(\q, t)$ remains the same as in proof of Lemma \ref{lem:marginalrenyi}, but the second term $F_2$ is
    \begin{align*}
        F_2 &=\q\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-1} \divR{(\rhO_{t}\Expec{}{\graD{\Loss_\D(\thet_{\step\kk})}|\ptheta_t})}\dif{\ptheta_t} \\
            &\quad -(\q-1)\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q} \divR{(\rhO_{t}'\Expec{}{\graD{\Loss_{\D}'(\thet_{\step\kk}')}|\ptheta_t})}\dif{\ptheta_t} \\
            &= (\q-1)\int_{\thetaspace}\dotP{\graD{\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q}}}{\rhO_{t}' \underbrace{\Expec{}{\graD{\Loss_{\D'}(\thet_{\step\kk}')}|\ptheta_t}}_{= G'(\ptheta_t)}}\dif{\ptheta_t} \\
            &\quad -\q\int_{\thetaspace}\dotP{\graD{\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-1}}}{\rhO_{t}\underbrace{\Expec{}{\graD{\Loss_\D(\thet_{\step\kk})}|\ptheta_t}}_{= G(\ptheta_t)}}\dif{\ptheta_t}
            \tag{From \eqr{eqn:divr_dotp_eq}} \\
            &= \q(\q-1)\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\dotP{\graD{\frac{\rhO_{t}}{\rhO_{t}'}}}{\frac{\rhO_{t}}{\rhO_{t}'}G'(\ptheta_t)}\rhO_t'\dif{\ptheta_t}\\
            &\quad -\q(\q-1)\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\dotP{\graD{\frac{\rhO_{t}}{\rhO_{t}'}}}{\frac{\rhO_{t}}{\rhO_{t}'}G(\ptheta_t)}\rhO_t'\dif{\ptheta_t} \\
            &= \q(\q-1)\int_{\thetaspace}\negthickspace\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\negthickspace\negthickspace\dotP{\negthickspace\graD{\frac{\rhO_{t}}{\rhO_{t}'}}}{\frac{\rhO_{t}}{\rhO_{t}'}\left(G'(\ptheta_t) - G(\ptheta_t)\right)\negthickspace}\rhO_t'\dif{\ptheta_t}
    \end{align*}
    Applying the trick (\eqr{eqn:young_ineq} with $b=2\gamma\tnoise^2$), we get
    \begin{align*}
        F_2 &\leq \gamma\tnoise^2 \q(\q-1)\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\norm{\graD{\frac{\rhO_{t}}{\rhO_{t}'}}}^2\rhO_{t}'\dif{\ptheta_t} \\
            &\quad + \frac{1}{\gamma}\frac{\q(\q-1)}{4\tnoise^2}\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\norm{\frac{\rhO_{t}}{\rhO_{t}'}\left(G'(\ptheta_t) - G(\ptheta_t)\right)}^2\rhO_{t}'\dif{\btheta} \\
            &\leq \gamma\tnoise^2 \q(\q-1) I(\q,t) + \frac{1}{\gamma}\frac{\q (\q-1)S_g^2}{4\tnoise^2\size^2(1-\step\be)^2} E(\q,t)
    \end{align*}
    Note that last inequality is from Lemma \ref{lem:new_delayed_loss_diff}, and the condition ${\step \leq \frac{1}{\smh}}$, which gives ${\vert\vert G(\ptheta_t) - G'(\ptheta_t)\vert\vert_2^2 \leq \frac{S_g^2}{\size^2(1-\step\be)^2}}$. We also substiute the integrals based on definitions in \eqr{eqn:frenyi_divergence} and \eqr{eqn:grenyi_divergence}.
    Finally, just like in Lemma \ref{lem:marginalrenyi} we get
    \begin{align*}
        \doh{R(\q,t)}{t}&=\frac{1}{\q-1}\times \frac{1}{E(\q,t)}\times\doh{E(\q,t)}{t}\\
                        &\leq -\gamma\tnoise^2 \q\frac{I(\q,t)}{E(\q,t)} + \frac{1}{\gamma}\frac{\q S_g^2}{4\tnoise^2\size^2(1-\step\be)^2} 
    \end{align*}
\end{proof}



    % \begin{reptheorem}{thm:RDbounddiscrete}[RDP for noisy GD under $\alp$-LSI]
    %      %
    % Let $\{\thet_t\}_{t\geq0}$ be the tracing diffusion for $\algo_{\text{Noisy-GD}}$ on dataset $\database$. Assume the loss function $\loss{\x}{\ptheta}$ is $\be$-smooth and total gradient $g(\ptheta;\D)$ has a finite sensitivity $\sen{\g}$. 
    
    % If for any $\D$, the distribution of $\thet_{t}$ satisfies $\alp$-LSI throughout ${0\leq t\leq \step\K}$, and the update step-size $\step< \frac{1}{\be}$, then $\algo_{\text{Noisy-GD}}$ satisfies $(\q, \eps)$ R\'enyi DP for
    % %
    % \begin{equation} 
    %     \eps \geq \frac{\q \sen{\g}^2}{2\alp\sig^4\size^2(1-\step\be)^2}(1-e^{-\sig^2\alp\step\K})
    % \end{equation}
    % \end{reptheorem}
    
    % \begin{proof}
    %     For every time interval ${\kk\step\leq t<(\kk+1)\step}$, the same PDE \eqr{eqn:evolvePDEdiscrete} applies under the stated assumptions. Therefore, we can solve the PDE directly for the entire duration $0 \leq t \leq \K\step$ almost identically as the proof of theorem \ref{thm:RDboundCD}, with a slight modification that constant ${a_2=\frac{\sen{\g}^2}{2\alp\sig^4\size^2(1-\step\be)^2}}$. This results in an RDP guarantee for noisy GD.
    % \end{proof}

\begin{reptheorem}{thm:RDbounddiscrete}
    %
    Let $\{\thet_t\}_{t\geq0}$ be the tracing diffusion for $\algo_{\text{Noisy-GD}}$ on dataset $\database$. Let $\loss{\x}{\ptheta}$ be a $\be$-smooth loss function on closed convex set $\C$, with a finite total gradient sensitivity $\sen{\g}$. 
    %
    If $\thet_{t}$ satisfies $\alp$-LSI throughout ${0\leq t\leq \step\K}$, and the step-size $\step< \frac{1}{\be}$, then $\algo_{\text{Noisy-GD}}$ satisfies $(\q, \eps)$ R\'enyi Differential Privacy for
    %
    \begin{equation} \label{eqn:RDbounddiscrete}
        \eps = \frac{\q \sen{\g}^2}{2\alp\sig^4\size^2(1-\step\be)^2}(1-e^{-\sig^2\alp\step\K})
    \end{equation}
\end{reptheorem}

\begin{proof}
    % The proof is similar to similar to that of Theorem~\ref{thm:RDboundCD} for coupled diffusion under the same finite total gradient sensitivity $S_g$ and $\alp$-LSI condition, except for dealing with the projection step. We only provide a sketch of proof. 
    
    The RDP evolution equation ~\ref{eqn:evolvePDEdiscrete} holds for projected noisy GD during the tracing diffusion in every time piece $\step\kk\leq t<\step(\kk+1)$. Therefore, we have

    \begin{equation*}
        \doh{R(\q,t)}{t} 
        \leq
        \frac{1}{\gamma}\frac{\q \sen{\g}^2}{4\tnoise^2\size^2(1-\step\be)^2}
        - 2(1-\gamma)\sig^2\alp \left[ \frac{R(\q,t)}{\q}     
        + (\q-1)\frac{\partial R(\q,t)}{\partial\q} \right]
    \end{equation*}
    
    Let $a_1=2(1-\gamma)\sig^2\alp$, ${a_2=\frac{1}{\gamma}\frac{S_g^2}{4\sig^2n^2(1-\step\be)^2}}$, $y=log(\q-1)$, and ${u(t,y)=\frac{R(\q,t)}{\q}-\frac{a_2}{a_1}}$.  We re-write \eqr{eqn:EvolvePDE} as the following form of transport with decay PDE
	%
	\begin{equation*}
	\frac{\partial u}{\partial t}+a_1 u+a_1\frac{\partial u}{\partial y}\leq 0,
	\end{equation*}
	%
	with initial condition $u(\step\kk,y)=\frac{R(\q,\step\kk)}{\q}-\frac{a_2}{a_1}$. By introducing variables $\tau=t$, and $z=t-\frac{1}{a_1} y$ and writing $v(\tau,z)=u(t,y)$, we get $\frac{\partial v}{\partial \tau}+a_1 v\leq0$, with initial condition ${v(\step\kk,z) = u(\step\kk,-a_1 (z-\step\kk))}$.  For every $z$, this means that the decay of $v$ is proportional to its present value. The solution for this problem is ${v(\tau,z) \leq v(\step\kk,z)e^{-a_1 (\tau-\step\kk)}}$.  By bringing back the original variables, we have
	%
	\begin{equation*}
	u(t,y)\leq u(\step\kk,y-a_1 (t-\step\kk))e^{-a_1 (t-\step\kk)}.
	\end{equation*}
	
	Further bringing back the original $R(\q,t)$ variables, we have
	%
	\begin{align*}
	R(\q,t)-\frac{a_2}{a_1}\q&\leq (R(\q,\step\kk)-\frac{a_2}{a_1}\q)e^{-a_1 (t-\step\kk)}\\
	\end{align*}

    Taking limit $t\rightarrow\step(\kk+1)$, where $\step\kk\leq t<\step(\kk+1)$, we have
    \begin{align*}
        \lim_{t\rightarrow\step(\kk+1)}R(\q,t)-\frac{a_2}{a_1}\q&\leq (R(\q,\step\kk)-\frac{a_2}{a_1}\q)e^{-a_1 \step}\\
    \end{align*}

    Because $\thet_{\step(\kk+1)}=\proj{\C}{\lim_{t\rightarrow\step(\kk+1)}\thet_t}$, and projection is post-processing which preserves privacy, 
    \begin{equation*}
        R(\q,\step(\kk+1))-\frac{a_2}{a_1}\q\leq \lim_{t\rightarrow\step(\kk+1)}R(\q,t)-\frac{a_2}{a_1}\q
    \end{equation*}
    
    Combining the above two inequalities, we immediately have the following recursive equation,
    \begin{equation*}
        R(\q,\step(\kk+1))-\frac{a_2}{a_1}\q\leq(R(\q,\step\kk)-\frac{a_2}{a_1}\q)e^{-a_1 \step}\\
    \end{equation*}
    
    Repeating this step for $\kk=0,\cdots,\K-1$ we have
    \begin{equation*}
        R(\q,\step\K)-\frac{a_2}{a_1}\q\leq(R(\q,0)-\frac{a_2}{a_1}\q)e^{-a_1 \step\K}\\
    \end{equation*}
    
    Because coupled tracing diffusion have the same start parameter, we have $R(\q,0)=0$.

    Therefore, taking the value $a_1=2(1-\gamma)\sig^2\alp$, ${a_2=\frac{1}{\gamma}\frac{S_g^2}{4\sig^2n^2(1-\step\be)^2}}$ into the equation, we have
    \begin{equation*}
        R(\q,\step\K)\leq \frac{\q \sen{\g}^2}{8\gamma(1-\gamma)\alp\sig^4\size^2(1-\step\be)^2}(1-e^{-2(1-\gamma)\sig^2\alp\step\K})
    \end{equation*}

    Setting $\gamma=\frac{1}{2}$ suffices to prove the R\'enyi privacy loss bound in the theorem.
\end{proof}
    
This R\'enyi differential privacy bound has quadratic dependence on the total gradient sensitivity $S_g$, which can upper bounded $S_g\leq 2\Lip$ when the loss function is $\Lip$-Lipschitz, which matches the RDP guarantees in the prior work~\cite{abadi2016deep, feldman2018privacy}.  As discussed before, here the convex set $\C$ is implicitly contrained to be bounded due to Lipschitzness and strong convexity. Morover, the strong convexity parameter $\lambda$ must be smaller than the smoothness parameter $\beta$ due to definition.



==> appendices/diffusion_proofs.tex <==
\section{Proofs for privacy analysis of Langevin Diffusion}
\label{sec:diffusion_proof}

\begin{replemma}{lem:marginalrenyi}[ Rate of R\'enyi Privacy Loss ]
%
Let $\loss{\x}{\ptheta}$ be a loss function on $\thetaspace$, with a finite total gradient sensitivity $\sen{\g}$. Then for coupled Langevin diffusions $\{\thet_t\}_{t\geq0}$ and $\{\thet_t'\}_{t\geq0}$ on neighboring datasets $\D, \D' \in \Domain$, under loss ${\smaloss{\x}{\ptheta}}$ and noise variance $\tnoise^2$, the R\'enyi privacy loss rate at any $t\geq0$ is upper bounded by
%
\begin{equation}
    \doh{\Ren{\q}{\thet_{t}}{\thet_{t}'}}{t}
    \leq 
    \frac{1}{\gamma}\frac{\q S_g^2}{4\tnoise^2\size^2}
    -
    (1-\gamma)\tnoise^2\q \frac{\Gren{\q}{\thet_{t}}{\thet_{t}'}}{\Fren{\q}{\thet_{t}}{\thet_{t}'}}.
\end{equation}
where $\gamma>0$ is a tuning parameter that we can fix arbitrarily according to our need.
\end{replemma}

\begin{proof}
    For brevity, let the functions ${R(\q,t)=\Ren{\q}{\rhO_{t}}{\rhO_{t}'}}$, ${E(\q,t)=\Fren{\q}{\rhO_{t}}{\rhO_{t}'}}$, and ${I(\q,t)=\Gren{\q}{\rhO_{t}}{\rhO_{t}'}}$. Under the stated assumptions $\doh{E(\q,t)}{t}$ is bounded as follows.
    \begin{align*}
        \doh{E(\q,t)}{t} &=\doh{}{t}\int_{\thetaspace}\frac{\rhO_{t}^{\q}}{\rhO_{t}'^{\q-1}}\dif{\ptheta} \\
        &= \q \int_{\thetaspace} \doh{\rhO_{t}}{t} \left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-1}\dif{\ptheta} \\
        &\quad    -(\q-1) \int_{\thetaspace} \doh{\rhO_{t}'}{t} \left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q} \dif{\ptheta} \\
        &=\ \q\int_{\thetaspace} \left(\tnoise^2\lapL{\rhO_{t}} + \divR{(\rhO_{t}\graD{\Loss(\D)})}\right)
            \left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-1}\dif{\ptheta} \\
        &\quad -(\q-1)\int_{\thetaspace} \big(\tnoise^2\lapL{\rhO_{t}'}+ \divR{(\rhO_{t}'\graD{\Loss(\D')})}\big) \\
        & \quad\quad\quad\quad\quad\quad\quad\quad\quad
            \left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^\q\dif{\ptheta}
            \tag{From \eqr{eqn:fokkerplanck}} \\
        &   \begin{rcases}
                =\tnoise^2 \q\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-1}\lapL{\rhO_{t}}\dif{\ptheta} \\
                \quad -\tnoise^2(\q-1)\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q}\lapL{\rhO_{t}'}\dif{\ptheta}
            \end{rcases} \eqdef F_1 \\
        &   \begin{rcases}  
                \quad +\q\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-1} \divR{(\rhO_{t}\graD{\Loss(\D)})}\dif{\ptheta} \\
                \quad -(\q-1)\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q} \divR{(\rhO_{t}'\graD{\Loss(\D')})}\dif{\ptheta}
            \end{rcases} \eqdef F_2
    \end{align*}
    Now $F_1$ is equivalent to the following.
    \begin{align*}
        F_1 &= \tnoise^2(\q-1)\int_{\thetaspace}\dotP{\graD{\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^\q}}{\graD{\rhO_{t}'}}\dif{\ptheta} \\
            &\quad -\tnoise^2 \q\int_{\thetaspace}\dotP{\graD{\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-1}}}{\graD{\rhO_{t}}}\dif{\ptheta}
                \tag{From \eqr{eqn:lapl_dotp_eq}} \\
            &= \tnoise^2 \q(\q-1)\int_{\thetaspace} \negthickspace\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\negthickspace\negthickspace\dotP{\negthickspace\graD{\frac{\rhO_{t}}{\rhO_{t}'}}}
                {\frac{\rhO_{t}}{\rhO_{t}'^2}\graD{\rhO_{t}'} - \frac{\graD{\rhO_{t}}}{\rhO_{t}'}\negthickspace}\rhO_{t}'\dif{\ptheta} \\
            &= -\tnoise^2 \q(\q-1)\Expec{\rhO_{t}'}{\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2} \norm{\graD{\frac{\rhO_{t}}{\rhO_{t}'}}}^2}
                \tag{$\because \graD{\frac{\rhO_{t}}{\rhO_{t}'}} = \frac{\graD{\rhO_{t}}}{\rhO_{t}'} - \frac{\rhO_{t}}{\rhO_{t}'^2}\graD{\rhO_{t}'}$} \\
            &= -\tnoise^2 \q(\q-1) I(\q, t) \tag{From \eqr{eqn:grenyi_divergence}}
    \end{align*}
    And $F_2$ is upper bounded by the following.
    \begin{align*}
        F_2 &= (\q-1)\int_{\thetaspace}\dotP{\graD{\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q}}}{\rhO_{t}' \graD{\Loss(\D')}}\dif{\ptheta} \\
            &\quad -\q\int_{\thetaspace}\dotP{\graD{\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-1}}}{\rhO_{t}\graD{\Loss(\D)}}\dif{\ptheta}
                \tag{From \eqr{eqn:divr_dotp_eq}} \\
            &= \q(\q-1)\negthickspace\int_{\thetaspace}\negthickspace\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\negthickspace\negthickspace\dotP{\negthickspace\graD{\frac{\rhO_{t}}{\rhO_{t}'}}}
                {\frac{\rhO_{t}}{\rhO_{t}'}\graD{\left(\Loss(D') - \Loss(D)}\right)\negthickspace}\rhO_{t}'\dif{\ptheta} \\
            &\leq \gamma \q(\q-1)\tnoise^2\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\norm{\graD{\frac{\rhO_{t}}{\rhO_{t}'}}}^2\rhO_{t}'\dif{\ptheta}
                \tag{From \eqr{eqn:young_ineq} with $b=2\gamma\tnoise^2$} \\
            &\quad + \frac{\q(\q-1)}{4\gamma\tnoise^2}\left(\frac{S_g}{\size}\right)^2\int_{\thetaspace}\left(\frac{\rhO_{t}}{\rhO_{t}'}\right)^{\q-2}\norm{\frac{\rhO_{t}}{\rhO_{t}'}}^2\rhO_{t}'\dif{\ptheta}
                \tag{$\because {\vert\vert\graD{\smaloss{\x}{\ptheta}}-\graD{\smaloss{\x'}{\ptheta}}\vert\vert_2\leq S_g}$ by definition} \\
            &\leq \gamma\tnoise^2 \q(\q-1) I(\q,t) + \frac{1}{\gamma}\frac{\q(\q-1)S_g^2}{4\tnoise^2\size^2} E(\q,t) \tag{From \eqr{eqn:frenyi_divergence} \& \eqr{eqn:grenyi_divergence}}
    \end{align*}
    Therefore, we get the following bound on the rate of Renyi divergence.
    \begin{align*}
        \doh{R(\q,t)}{t}&=\frac{1}{\q-1}\times \frac{1}{E(\q,t)}\times\doh{E(\q,t)}{t}\\
                                                &\leq -(1-\gamma)\tnoise^2 \q\frac{I(\q,t)}{E(\q,t)} + \frac{1}{\gamma}\frac{\q S_g^2}{4\tnoise^2\size^2} 
    \end{align*}
\end{proof}

\begin{replemma}{lem:RDinLSI}[ $\alp$-LSI in terms of Rényi Divergence~\cite{vempala2019rapid} ]
    %
    Suppose $\rhO,\rhO'$ are probability distributions of random variables $\thet_t, \thet_t'$ on $\thetaspace$. If $\frac{\rhO}{\rhO'}\in\Ftheta{\thet_t'}$, 
    then for any $\q \geq 1$, 
    %
    \begin{align*} 
        \Ren{\q}{\thet_t}{\thet_t'} 
        + 
        \q(\q - 1) \doh{\Ren{\q}{\thet_t}{\thet_t'}}{\q}  
        \leq 
        \frac{\q^2}{2\alp} \frac{\Gren{\q}{\thet_t}{\thet_t'}}{\Fren{\q}{\thet_t}{\thet_t'}},
    \end{align*}
    if and only if $\rhO'$ satisfies $\alp$-LSI.
\end{replemma}

\begin{proof}
    For brevity, let the functions ${R(\q)=\Ren{\q}{\thet_t}{\thet_t'}}$, ${E(\q)=\Fren{\q}{\thet_t}{\thet_t'}}$, and ${I(\q)=\Gren{\q}{\thet_t}{\thet_t'}}$. 
    Let function ${g^2(\ptheta)=\left(\frac{\rhO(\ptheta)}{\rhO'(\ptheta)}\right)^\q}$. Then,
    \begin{align*}
        \Expec{\rhO'}{g^2} = \Expec{\rhO'}{\left(\frac{\rhO}{\rhO'}\right)^{\q}} = \Frenyi{\q}{\rhO}{\rhO'},
        \tag{From \eqr{eqn:frenyi_divergence}}
    \end{align*}
    and,
    \begin{align*}
        \Expec{\rhO'}{g^2 \log g^2} &= \Expec{\rhO'}{\left(\frac{\rhO}{\rhO'}\right)^{\q} 
                                   \log \left(\frac{\rhO}{\rhO'}\right)^{\q}} \\
                                   &= \q \doh{}{\q}\Expec{\rhO'}{\int_{\q}\left(\frac{\rhO}{\rhO'}\right)^{\q} 
                                   \log\left(\frac{\rhO}{\rhO'}\right)\dif{\q}}
                                   \tag{Lebniz's rule} \\
                                   &= \q \doh{}{\q}\Expec{\rhO'}{\left(\frac{\rhO}{\rhO'}\right)^{\q}}
                                   = \q \doh{E(\q)}{\q}
                                   \tag{From \eqr{eqn:frenyi_divergence}}
    \end{align*}
    Moreover,
    \begin{align*}
        \Expec{\rhO'}{\norm{\graD{g}}^2} = \Expec{\rhO'}{\norm{\graD{
        \left(\frac{\rhO}{\rhO'}\right)^\frac{\q}{2}}}^2}
        = \frac{\q^2}{4} I(\q)
        \tag{From \eqr{eqn:grenyi_divergence}}
    \end{align*}
    Substituting \eqr{eqn:lsi_standard} with the above equalities give
    \begin{align*}
            &\Ent{\rhO'}{g^2} \leq \frac{2}{\alp} \Expec{\rhO'}{\norm{\graD{g}}^2} \\
        \iff&\q\doh{E(\q)}{\q} - E(\q) \log E(\q)
            \leq \frac{\q^2}{2\alp} I(\q) \\
        \iff&\q\doh{\log E(\q)}{\q} - \log E(\q) 
            \leq \frac{\q^2}{2\alp} \frac{I(\q)}{E(\q)} \\
        \iff&\q\doh{}{\q}\left((\q-1) R(\q)\right) - (\q - 1)R(\q)
            \leq \frac{\q^2}{2\alp} \frac{I(\q)}{E(\q)}
            \tag{From \eqr{eqn:renyi_divergence}} \\
	\iff& R(\q) + \q(\q-1)\doh{R(\q)}{\q}
            \leq \frac{\q^2}{2\alp} \frac{I(\q)}{E(\q)}
    \end{align*}
\end{proof}


\begin{reptheorem}{thm:linearRDP}
	Let $\loss{\x}{\ptheta}$ be a loss function on $\thetaspace$, with a finite total gradient sensitivity $\sen{\g}$, then the Langevin diffusion under loss $\ell(\theta;\x)$ and noise variance $\sig^2$ for time $T$ satisfies $(\alpha,\eps)$-RDP for $\eps=\frac{\alpha S_g^2 T}{4\sig^2\size^2}$.
\end{reptheorem}
\begin{proof}
    Setting $\gamma=1$ in Lemma~\ref{lem:marginalrenyi} gives constant privacy loss rate. Integrating over $t$ suffices.
\end{proof}



\begin{theorem}[RDP for Langevin Diffusion under $\alp$-LSI]
    \label{thm:RDboundCD}
	%
    For a given dataset $\database \in \Domain$ and any $t>0$, let $\{\thet_t\}_{t\geq 0}$ be the Langevin diffusion on $\database$ for loss function ${\smaloss{\x}{\ptheta}}$ and variance~$\sig^2$.  If the distribution of $\thet_{t}$ satisfies $\alp$-LSI, for any~$\database$ and any $0\leq t\leq T$, the algorithm corresponding to the Langevin diffusion satisfies $(\q,\eps)$-RDP for
    %
    \begin{equation} 
        \eps = \frac{\q S_g^2}{2 \alp n^2 \sig^4}(1-e^{-\sig^2\alp T})
    \end{equation}
    %
    where $\sen{\g}$ is the finite sensitivity of total gradient ${\g(\ptheta; \D) = \sum_{\x \in \D} \graD{\loss{\x}{\ptheta}}}$.
\end{theorem}

\begin{proof}
	Let $a_1=2(1-\gamma)\sig^2\alp$, ${a_2=\frac{1}{\gamma}\frac{S_g^2}{4n^2\sig^2}}$, $y=log(\q-1)$, and ${u(t,y)=\frac{R(\q,t)}{\q}-\frac{a_2}{a_1}}$.  We re-write \eqr{eqn:EvolvePDE} as the following form of transport with decay PDE
	%
	\begin{equation*}
	\frac{\partial u}{\partial t}+a_1 u+a_1\frac{\partial u}{\partial y}\leq 0,
	\end{equation*}
	%
	with initial condition $u(0,y)=-\frac{a_2}{a_1}$. By introducing variables $\tau=t$, and $z=t-\frac{1}{a_1} y$ and writing $v(\tau,z)=u(t,y)$, we get $\frac{\partial v}{\partial \tau}+a_1 v\leq0$, with initial condition ${v(0,z) = u(0,-a_1 z)}$.  For every $z$, this means that the decay of $v$ is proportional to its present value. The solution for this problem is ${v(\tau,z) \leq v(0,z)e^{-a_1 \tau}}$.  By bringing back the original variables, we have
	%
	\begin{equation*}
	u(t,y)\leq u(0,y-a_1 t)e^{-a_1 t}.
	\end{equation*}
	
	Therefore,
	%
	\begin{align*}
	R(\q,t)&\leq \frac{a_2}{a_1}(1-e^{-a_1 t})\\
    &=\frac{\q S_g^2}{8\gamma(1-\gamma) \alp n^2 \sig^4}(1-e^{-\sig^2\alp T})\\
    &=\frac{\q S_g^2}{2 \alp n^2 \sig^4}(1-e^{-\sig^2\alp T})\quad\text{set }\gamma=\frac{1}{2}.
	\end{align*}
\end{proof}



==> appendices/smoothness.tex <==
\section{Relaxing smoothness in Discretization}

Firstly, I derive a analogy lemma of Lemma~\ref{lem:new_delayed_loss_diff} which does not require smoothness of loss function.

\begin{lemma}
    \label{lem:nonsmooth_delayed_loss_diff}
    Let $\D, \D' \in \Domain$ be neighboring datasets of size $\size$. Let loss function  $\loss{\x}{\ptheta}$ be $\smh$-smooth, and sum of loss gradients $g(\ptheta;\D)=\sum_{\x_i\in\D}\nabla\ell(\ptheta;\x_i)$ has finite sensitivity $S_g$.
     For any $\tnoise^2$ and $\step$, given a sample $\thet_t \in \thetaspace$ at any time $t\geq0$, let r.v.'s $\thet_{\step\kk}, \thet_{\step\kk}', \thet_t, \thet_t'$ satisfy
    \begin{align}
        \label{eqn:new_delayed_update}
        \thet_{\step\kk} - (t-\step\kk) \graD{\Loss_\D(\thet_{\step\kk})} + \sqrt{2t\tnoise^2}\Z = \thet_t, \\
        \thet_{\step\kk}' - (t-\step\kk) \graD{\Loss_{\D'}(\thet_{\step\kk}')} + \sqrt{2t\tnoise^2}\Z' = \thet_t',
    \end{align}
    where $\Z, \Z' \sim \Gaus{0}{\Id}$, and $\kk$ is an integer s.t. ${\step\kk \leq t \leq \step(\kk+1)}$. Then, given $\ptheta_t$ was observed at time $t$, i.e. ${\thet_t = \thet_t' = \ptheta_t}$,
    \begin{align}
        \label{eqn:newdiscrete_error}
        \Big\Vert\Expec{}{\graD{\Loss_{\D}(\thet_{\step\kk})}\vert\ptheta_t} - &\Expec{}{\graD{\Loss_{\D'}(\thet_{\step\kk}')}\vert\ptheta_t}\Big\Vert_2^2 \leq \frac{S_g^2}{n^2(1-\step\be)^2}.
    \end{align}
\end{lemma}

==> sections/tablecompare.tex <==
% !TEX root = ../main.tex

    \centering
    
    \begin{tabular}{|l||c|l|l|l|}
            \hline
            \bfseries Privacy Analysis & \bfseries Algorithm & \bfseries $\eps$ in $(\eps,\del)$-DP & \bfseries $\eps$ in $(\q,\eps)$-RDP & \bfseries Assumptions\\
            \hline
            \hline
        % 
            \citet{bassily2014private} & GD & $\frac{\Lip}{\sig}\sqrt{\K\log(\K/\del)log(1/\del)}$& -- &$\Lip$-Lipschitz \\[0.1cm]
            \hline
            \citet{abadi2016deep} & SGD  & $\frac{\Lip}{\sig}\sqrt{\frac{b}{\size}\K log(1/\del)}$& -- &gradients clipped to $\Lip$ \\[0.1cm]
            \hline
            \citet{feldman2018privacy} & SGD  & $\frac{\Lip}{\sig}\sqrt{\frac{1}{\size}\K log(1/\del)}$ &$\frac{\Lip^2\K\q}{\tnoise^2 n}$ &convex, $\smh$-smooth, and $\Lip$-Lipschitz \\[0.1cm]
            \hline
            \citet{balle2019privacy} & SGD & $\frac{\Lip}{\sig}\sqrt{\frac{\K log(1/\del)}{\size-1}(1-\frac{2\step\be\lam}{\be+\lam})^{\frac{\size}{2}}}$ & $\frac{\Lip^2\K\q}{\sig^2(\size-1)}(1-\frac{2\step\be\lam}{\be+\lam})^{\frac{\size}{2}}$&$\lam$-strongly convex, $\Lip$-Lipschitz, and $\be$-smooth \\[0.1cm]
            \hline
            This Paper & GD & $\frac{S_g}{\sig\size}\sqrt{\frac{log(1/\del)}{\lam}(1-e^{-\lam\step\K/2})}$ & $\frac{\q S_g^2}{\lam\sig^2 n^2}(1-e^{-\lam \step\K/2})$&$\lam$-strongly convex and $\be$-smooth, \\
            & & & & finite sensitivity $S_g$ for total gradient \\[0.1cm]
            \hline
            \multicolumn{5}{p{{0.93\linewidth}}}{Comparison of $\eps$ in $(\eps,\del)$-differential privacy and $(\q, \eps)$-R\'enyi differential privacy for noisy gradient descent variants, using different differential privacy accounting techniques. Size of input dataset is $\size$, and the (expected) number of iterations (as passes over the \emph{whole} dataset) is $\K$. Noise variance across the algorithms is $\tnoise^2$ and learning rate is $\step$. For \citet{abadi2016deep}, mini-batches of size $b$ are sampled via Poisson sub-sampling with Bernoulli probability $b/\size$.  We ignore the numerical constants in the bounds.}
        \end{tabular}
